SINCERE: Supervised Information Noise-Contrastive Estimation REvisited

The information noise-contrastive estimation (InfoNCE) loss function provides the basis of many self-supervised deep learning methods due to its strong empirical results and theoretic motivation. Previous work suggests a supervised contrastive (SupCon) loss to extend InfoNCE to learn from available class labels. This SupCon loss has been widely-used due to reports of good empirical performance. However, in this work we find that the prior SupCon loss formulation has questionable justification because it can encourage some images from the same class to repel one another in the learned embedding space. This problematic intra-class repulsion gets worse as the number of images sharing one class label increases. We propose the Supervised InfoNCE REvisited (SINCERE) loss as a theoretically-justified supervised extension of InfoNCE that eliminates intra-class repulsion. Experiments show that SINCERE leads to better separation of embeddings from different classes and improves transfer learning classification accuracy. We additionally utilize probabilistic modeling to derive an information-theoretic bound that relates SINCERE loss to the symmeterized KL divergence between data-generating distributions for a target class and all other classes.

==> Makefile <==
## To build paper PDF: 'make main.pdf'

SHELL=/bin/bash

MAIN?=main
MAINDOCX?=maindocx

STYLE_FILE=jmlr.cls

FIG_DIR=images/

TEX_FILES_EXCEPT_MAIN=$$(bash -c "find . -name '*.tex' -maxdepth 1 | sort -n | grep -v ${MAIN}.tex")
TMP_RESULT=$$(bash -c "find . -name '*.tex' -maxdepth 1 | xargs grep ${FIG_DIR} | cut -d':' -f2 | grep -v '%'");
PDF_FIG_FILES=$$(python -c "print(' '.join([s + ('.pdf' * (1 - s.endswith('.pdf')) * (1 - s.endswith('.png'))) for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('''${FIG_DIR}''')]))")
PNG_FIG_FILES=$$(python -c "print(' '.join([s for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('''${FIG_DIR}''') and s.endswith('.png') ]))")
JPG_FIG_FILES=$$(python -c "print(' '.join([s for s in [x.partition('}')[0] for x in '''${TMP_RESULT}'''.split('{')] if s.startswith('''${FIG_DIR}''') and s.endswith('.jpg') ]))")

OUTPUTFILE_DOCX?=$(MAIN).docx
BIBLIO_OPTS = --bibliography *.bib --csl apa.csl

all: $(MAIN).pdf $(MAIN).docx

clean:
	rm -fv *.zip *.aux *.log *.bbl *.blg *.ptc *.toc *.out *.lot *.lof *.dvi *.ps *.pdf *.docx

clean_extras:
	rm -fv *.aux *.bbl *.blg *.toc *.out *.lot *.lof

pdf: $(MAIN).pdf

paper: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).bbl *.tex sections/*.tex
	# Run 3x to get cross refs right
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) || true
	pdflatex -interaction nonstopmode $(MAIN) && rm -fv *.aux *.blg *.toc *.out *.lot *.lof

$(MAIN).bbl: $(MAIN).tex *.tex *.bib sections/*.tex
	pdflatex -interaction nonstopmode $(MAIN) || true
	bibtex $(MAIN) && rm $(MAIN).pdf


$(OUTPUTFILE_DOCX): $(STYLE_FILE) *.tex *.bib ${FIG_DIR}/*.png
	pandoc $(MAINDOCX).tex \
		--from latex \
		--to docx \
		--output $(OUTPUTFILE_DOCX) \
		$(BIBLIO_OPTS)

src_for_arxiv.zip: $(MAIN).bbl $(MAIN).tex *.tex *.bib
	zip -r src_for_arxiv.zip \
		*.bbl \
		$(MAIN).tex \
		$(STYLE_FILE) \
		$(TEX_FILES_EXCEPT_MAIN) \
		$(PDF_FIG_FILES) \
		$(PNG_FIG_FILES) \
		$(JPG_FIG_FILES)


==> cover_letter/cover_letter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``SINCERE: Supervised Information Noise-Contrastive Estimation REvisited'' to the \emph{Journal of Machine Learning Research}.

Our manuscript provides new theoretical and empirical knowledge about supervised contrastive learning. We examine an existing popular loss for supervised contrastive learning, the ``SupCon'' loss by Khosla et al., and show it has a problematic issue: intra-class repulsion. We then revisit the theoretic motivation of the self-supervised InfoNCE loss and use this to derive a novel loss we call SINCERE which avoids intra-class repulsion.
Experiments show that our SINCERE loss eliminates problematic intra-class repulsion found in the previous loss, improves the desired separation of noise and target classes, and ultimately improves transfer learning performance. We further provide an information-theoretic bound relating our SINCERE loss to a symmeterized KL divergence between data-generating distributions for target and noise clsases.

This paper does not significantly overlap with any previous publications by the authors.

We suggest the following action editors and referees for our submission.

Suggested Action Editors:
\begin{itemize}
    \item Stefanie Jegelka, Massachusetts Institute of Technology (stefje@csail.mit.edu)
    \item Benjamin Marlin, University of Massachusetts Amherst (marlin@cs.umass.edu)
    \item Fei Sha, Google (fsha@google.com)
    \item Genevera Allen, Rice University (gallen@rice.edu)
    % https://academic.oup.com/biometrics/article/79/4/3846/7587579
    \item Quentin Berthet, Google DeepMind (qberthet@google.com)
    % https://arxiv.org/pdf/2211.10420
\end{itemize}

Suggested Reviewers:
\begin{itemize}
    \item Laurence Aitchison, University of Bristol (laurence.aitchison@bristol.ac.uk)
    % work on understanding InfoNCE as a probabilistic model: https://arxiv.org/pdf/2107.02495
    \item Dilip Krishnan, Google (dilipkay@gmail.com)
    % last author on SupCon paper
    \item Eric Nalisnick, Johns Hopkins University (nalisnick@jhu.edu)
    % solid probabilistic modeler, will appreciate the ideas I think, listed as a JMLR reviewer
    \item Richard Radke, Rensselaer Polynechnic Institute ( rjradke@ecse.rpi.edu)
    % vision + contrastive learning, with some probabilistic methods too
    \item Cedric Archambeau, Helsing.AI (cedric.archambeau@helsing,ai)
    % another solid probabilistic modeler listed as a JMLR reviewer
    % \item David Kristjanson Duvenaud, University of Toronto (duvenaud@cs.toronto.edu)
    % https://arxiv.org/pdf/1806.07366
    % also, see MetaLearning to improve pretraining for his contrastive expertise: https://proceedings.neurips.cc/paper/2021/file/c3810d4a9513b028fc0f2a83cb6d7b50-Paper.pdf
    %\item Edgar Dobriban, University of Pennsylvania (dobriban@wharton.upenn.edu)
    % https://arxiv.org/pdf/2310.07891
    %\item Kumar Avinava Dubey, Google Research (avinava.dubey@gmail.com)
    % https://arxiv.org/pdf/2310.13225

\end{itemize}

Our submission has the following keywords: contrastive learning, representation learning, probabilistic modeling, supervised learning, transfer learning.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Patrick Feeney (Tufts University)\\
Michael C. Hughes (Tufts University)

\end{document}








































==> scratch/notation_mismatch.tex <==
\todo{transposing p and S to better match Eq 13}

Current self-supervised (Should not change math, but explanation should explain $z_S$ as the $y_S$ representation)

$\ratpdf{x_S} \implies e^{f_\theta(x_S, y_S)} \implies e^{z_S \cdot z_S'}$

$\ratpdf{x_n} \implies e^{f_\theta(x_n, y_S)} \implies e^{z_S \cdot z_n}$

Current supervised ($z_S$ implied to be $x_S$ for the first but $y_S$ for the second)

$\ratpdf{x_S} \implies e^{f_\theta(x_S, y_S)} \implies e^{z_S \cdot z_p}$

$\ratpdf{x_n} \implies e^{f_\theta(x_n, y_S)} \implies e^{z_S \cdot z_n}$

Alternative supervised ($z_S$ is always $y_S$)

$\ratpdf{x_S} \implies e^{f_\theta(x_S, y_S)} \implies e^{z_p \cdot z_S}$

$\ratpdf{x_n} \implies e^{f_\theta(x_n, y_S)} \implies e^{z_n \cdot z_S}$

Alternative supervised 2 (also changing $f$ format)

$\ratpdf{x_S} \implies e^{f_\theta(x_p, x_S)} \implies e^{z_p \cdot z_S}$

$\ratpdf{x_n} \implies e^{f_\theta(x_n, x_S)} \implies e^{z_n \cdot z_S}$

Is the softmax valid given two choices of $S$ and a partner?
\begin{align}
1 &?
\frac{e^{z_1 \cdot z_p}}{e^{z_1 \cdot z_p} + e^{z_1 \cdot z_2}}
+ \frac{e^{z_2 \cdot z_p}}{e^{z_2 \cdot z_p} + e^{z_1 \cdot z_2}} \\
1 &?
\frac{e^{z_1 \cdot z_p}(e^{z_2 \cdot z_p} + e^{z_1 \cdot z_2})
+ e^{z_2 \cdot z_p}(e^{z_1 \cdot z_p} + e^{z_1 \cdot z_2})}
{(e^{z_1 \cdot z_p} + e^{z_1 \cdot z_2})(e^{z_2 \cdot z_p} + e^{z_1 \cdot z_2})} \\
1 &\neq
\frac{e^{z_1 \cdot z_p}e^{z_1 \cdot z_2}
+ 2e^{z_1 \cdot z_p}e^{z_2 \cdot z_p}
+ e^{z_2 \cdot z_p}e^{z_1 \cdot z_2}}
{e^{z_1 \cdot z_p}e^{z_2 \cdot z_p}
+ e^{z_1 \cdot z_p}e^{z_1 \cdot z_2}
+ e^{z_2 \cdot z_p}e^{z_1 \cdot z_2}
+ e^{z_1 \cdot z_2}e^{z_1 \cdot z_2}}
\end{align}

Is the softmax valid given two choices of $S$ and a partner when written in terms of similarity expectations?
\begin{align}
1 &?
\frac{e^{s(1, S)}}{e^{s(1, S)} + e^{s(n, S)}}
+ \frac{e^{s(2, S)}}{e^{s(2, S)} + e^{s(n, S)}} \\
\end{align}


==> sections/impact.tex <==
\section{Impact Statement}
% Authors are required to include a statement of the potential broader impact of their work, including its ethical aspects and future societal consequences. This statement should be in a separate section at the end of the paper (co-located with Acknowledgements, before References), and does not count toward the paper page limit. In many cases, where the ethical impacts and expected societal implications are those that are well established when advancing the field of Machine Learning, substantial discussion is not required, and a simple statement such as: 

This paper presents work whose goal is to advance supervised feature learning and classification.
There are many potential societal consequences of our work, with current methods impacting hiring \citep{drage2022does}, migration \citep{migration}, the production of social norms and biases \citep{kupriianova2023ai, buolamwini2018gender, mehrabi2021survey, leavy2018gender, UNESCO}, and much more.
We encourage responsible use of machine learning through methods such as those proposed by \citet{mitchell2019model}, \citet{gebru2021datasheets}, and \citet{prabhakaran2022human}.


==> tables/cos_sim_separate.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{l|ll|ll|ll|ll}
\toprule
              & \multicolumn{2}{c|}{CIFAR-2} & \multicolumn{2}{c|}{CIFAR-10} & \multicolumn{2}{c|}{CIFAR-100} & \multicolumn{2}{c}{ImageNet-100} \\
Training Loss & Target          & Noise        & Target          & Noise        & Target          & Noise        & Target          & Noise        \\ \midrule
SupCon        & 1.00         & 0.59        & 1.00         & 0.73         & 1.00          & 0.56         & 1.00           & 0.97          \\
SINCERE       & 1.00         & \textbf{0.03}        & 1.00         & \textbf{0.15}         & 0.98          & \textbf{0.52}         & 0.95           & \textbf{0.80}          \\
\bottomrule
\end{tabular}
\caption{
Median of test set nearest neighbors.
% SINCERE's performance is essentially indistinguishable from SupCon.
% No results are boldfaced, as differences are \emph{not} statistically significant according to bootstrap interval analysis.
}
\label{table:cos_sim}
\end{table*}
